Basis set extrapolation for post-CCSD(T) contributions reconsidered

Higher-order correlation contributions beyond CCSD(T) are a key ingredient of high-accuracy computational thermochemistry and spectroscopy approaches. In an attempt to more firmly rationalize their basis set convergence behavior, we have carried out benchmark studies for over three dozen molecules with basis sets through cc-pV7Z. Connected quadruples (Q) converge smoothly to the basis set limit if evaluated for at least cc-pVTZ basis sets; cc-pVDZ is anomalous for ionic systems. Post-CCSDT(Q) contributions converge quite rapidly with the basis set, with even a truncated cc-pVTZ(d) basis set yielding results near the basis set limit. In contrast, higher-order triples contributions, $T_3-(T)$, converge slowly and at times erratically: we show that this is the superposition of three different convergence behaviors, namely (a) CCSDT-3 $-$ CCSD(T) with leading term $E^{(5)}_{TQ}$ (moderately fast); (b) CCSDT $-$ CCSDT-4 (higher-order triples coupling terms, very fast); and (c) triples-on-triples ladder diagrams (slow) in CCSDT-4 $-$ CCSDT-3, with leading term $E^{(5)}_{TT}$. The slow convergence of the latter dominates for large basis sets. A Petersson-style $(L+a)^{-3}$ extrapolation well describes convergence behavior with different shifts $a=+1.10$ for CCSDT-3 $-$ CCSD(T), $a=+0.84$ for CCSDT $-$ CCSDT-3, $a=+0.69$ for combined CCSDT $-$ CCSD(T), and $a=-0.66$ for (Q).

==> tables/top-six.tex <==
\footnotesize
\setlength{\tabcolsep}{2.5pt}
\begin{tabular}[t]{@{}l*{6}{S[table-format=-1.3]}@{}}
\toprule
 & {BN} & {C$_2$} & {P$_2$} & {N$_2$O} & {O$_3$} & {NO$_2$} \\
\midrule
\multicolumn{7}{@{}l}{$[\textrm{CCSDT-3}]-[\textrm{CCSD(T)}]$} \\
VTZ & -0.712 & -2.297 & -0.709 & -0.270 & -0.903 & 0.070 \\
VQZ & -0.577 & -2.191 & -0.677 & -0.208 & -0.801 & 0.133 \\
V5Z & -0.518 & -2.147 & -0.642 & -0.170 & -0.739 & 0.175 \\
V6Z & -0.491 & -2.127 & -0.625 & -0.149 & -0.705 & 0.198 \\
V7Z & -0.476 & -2.116 & -0.614 & -0.136 & -0.684 & 0.212 \\
REF2$^{b}$ & -0.449 & -2.096 & -0.599 & -0.116 & -0.652 & 0.234 \\
REF1$^{c}$ & -0.448 & -2.095 & -0.593 & -0.112 & -0.645 & 0.238 \\
\midrule
\multicolumn{7}{@{}l}{$[\textrm{CCSDT}]-[\textrm{CCSDT-3}]$} \\
VTZ & -1.734 & 0.385 & -0.013 & -0.932 & -0.090 & -0.648 \\
VQZ & -1.978 & 0.085 & -0.166 & -1.175 & -0.423 & -0.900 \\
V5Z & -2.093 & -0.047 & -0.249 & -1.293 & -0.598 & -1.026 \\
V6Z & -2.148 & -0.108 & -0.302 & -1.350 & -0.681 & -1.085 \\
V7Z & -2.178 & -0.142 & -0.333 & -1.382 & -0.727 & -1.119 \\
REF2$^{b}$ & -2.234 & -0.203 & -0.384 & -1.439 & -0.810 & -1.177 \\
REF1$^{c}$ & -2.234 & -0.206 & -0.391 & -1.442 & -0.814 & -1.181 \\
\midrule
\multicolumn{7}{@{}l}{$[\textrm{CCSDT}]-[\textrm{CCSD(T)}]$} \\
VTZ & -2.446 & -1.912 & -0.722 & -1.202 & -0.993 & -0.578 \\
VQZ & -2.555 & -2.106 & -0.843 & -1.383 & -1.224 & -0.767 \\
V5Z & -2.611 & -2.194 & -0.891 & -1.463 & -1.337 & -0.851 \\
V6Z & -2.639 & -2.235 & -0.927 & -1.499 & -1.386 & -0.887 \\
V7Z & -2.654 & -2.258 & -0.947 & -1.518 & -1.411 & -0.906 \\
REF2$^{b}$ & -2.683 & -2.299 & -0.983 & -1.555 & -1.462 & -0.943 \\
REF1$^{c}$ & -2.682 & -2.301 & -0.985 & -1.554 & -1.458 & -0.943 \\
\bottomrule
\end{tabular}
\hfill
\begin{tabular}[t]{@{}l*{6}{S[table-format=-1.3]}@{}}
\toprule
 & {BN} & {C$_2$} & {P$_2$} & {N$_2$O} & {O$_3$} & {NO$_2$} \\
\midrule
\multicolumn{7}{@{}l}{$[(\textrm{Q})]=[\textrm{CCSDT(Q)}]-[\textrm{CCSDT}]$} \\
VTZ(d)$^{a}$ & 2.911 & 3.014 & 1.186 & 2.160 & 4.214 & 2.022 \\
VTZ & 3.026 & 3.220 & 1.431 & 2.259 & 4.383 & 2.123 \\
VQZ(f)$^{a}$ & 3.138 & 3.326 & 1.509 & 2.358 & 4.587 & 2.240 \\
VQZ & 3.173 & 3.352 & 1.567 & 2.380 & 4.621 & 2.261 \\
V5Z & 3.223 & 3.393 & 1.608 & 2.418 & 4.713 & 2.310 \\
V6Z & 3.240 & 3.407 & 1.625 & 2.430 & 4.747 & {---} \\
V7Z & 3.248 & 3.413 & 1.633 & {---} & {---} & {---} \\
REF2$^{b}$ & 3.266 & 3.429 & 1.651 & 2.449 & 4.800 & {---} \\
REF1$^{c}$ & 3.263 & 3.424 & 1.648 & {---} & {---} & {---} \\
\midrule
\multicolumn{7}{@{}l}{$[(\textrm{Q})_\Lambda]-[(\textrm{Q})]$} \\
VDZ & -0.722 & -0.490 & -0.064 & -0.159 & -0.495 & -0.160 \\
VTZ(d)$^{a}$ & -0.872 & -0.549 & -0.073 & -0.143 & -0.498 & -0.164 \\
VTZ & -0.843 & -0.572 & -0.081 & -0.145 & -0.514 & -0.168 \\
VQZ(f)$^{a}$ & -0.867 & -0.587 & -0.083 & -0.142 & -0.529 & -0.170 \\
VQZ & -0.866 & -0.591 & -0.085 & -0.140 & -0.530 & -0.168 \\
V5Z(f)$^{a}$ & -0.870 & -0.591 & -0.083 & -0.139 & -0.535 & -0.171 \\
REF3$^{d}$ & -0.869 & -0.595 & -0.084 & -0.137 & -0.535 & -0.168 \\
\midrule
\multicolumn{7}{@{}l}{$[\textrm{CCSDTQ}]-[\textrm{CCSDT(Q)}_\Lambda]$} \\
VDZ & -0.365 & -0.578 & -0.044 & -0.296 & -0.425 & -0.232 \\
VTZ(d)$^{a}$ & -0.339 & -0.570 & -0.061 & -0.298 & -0.463 & -0.236 \\
VTZ & -0.312 & -0.530 & -0.065 & -0.299 & -0.464 & -0.230 \\
VQZ(f)$^{a}$ & -0.316 & -0.534 & -0.074 & -0.319 & -0.508 & {---} \\
VQZ & -0.316 & -0.537 & -0.084 & {---} & {---} & {---} \\

REF4$^{e}$ & -0.319 & -0.537 & -0.076 & {---} & {---} & {---} \\
\bottomrule
\end{tabular}

\smallskip
\parbox{\textwidth}{\footnotesize
V$n$Z = cc-pV$n$Z. $^{a}$\,V$n$Z($l$): cc-pV$n$Z truncated at angular momentum $l$ (hydrogen one $l$ lower).
$^{b}$\,REF2: Riemann3 extrapolation from cc-pV\{5,6\}Z, $E_\infty = E_6 + 1.5548\,(E_6-E_5)$.
$^{c}$\,REF1: Riemann3 extrapolation from cc-pV\{6,7\}Z, $E_\infty = E_7 + 1.8805\,(E_7-E_6)$.
$^{d}$\,REF3 = cc-pV5Z(g). $^{e}$\,REF4 = cc-pV5Z(f). ---: not available or not presently feasible.}

